Agent-based modeling of a price information trading business

We describe an agent-based simulation of a fictional (but feasible) information trading business. The Gas Price Information Trader (GPIT) buys information about real-time gas prices in a metropolitan area from drivers and resells the information to drivers who need to refuel their vehicles. Our simulation uses real world geographic data, lifestyle-dependent driving patterns and vehicle models to create an agent-based model of the drivers. We use real world statistics of gas price fluctuation to create scenarios of temporal and spatial distribution of gas prices. The price of the information is determined on a case-by-case basis through a simple negotiation model. The trader and the customers are adapting their negotiation strategies based on their historical profits. We are interested in the general properties of the emerging information market: the amount of realizable profit and its distribution between the trader and customers, the business strategies necessary to keep the market operational (such as promotional deals), the price elasticity of demand and the impact of pricing strategies on the profit.

==> NotIncluded.tex <==
% *****************************************************
%
%   Discussion about the initial offer of the client
%
% *****************************************************

The GPIT is intelligent enough to make the deal terminate in a selfish
manner, which if it does then the agreement is of little benefit to
user. To overcome such large amount of money to be leeched by the
GPIT, the customer has a maximum limit on its initial offer, i.e.,
$c_{max}^{u}$. Hence, after several negotiations if the initial offer of
customer shifts to $c_{max}^{u}$, there is an automatic reduction in initial
offer to keep scenario somehow fair, i.e.,
\begin{algorithm}
\begin{algorithmic} 
\IF {$\mathcal{X}^{m-1}_{c \leftrightarrow s} : u^{c}_{min} \geq c^{u}_{max}$}
\WHILE  {$u^{c}_{min} << c^{u}_{max}$}
\STATE $u^{c}_{min} = u^{c}_{min} - u_{k}$
\ENDWHILE
\ENDIF
\end{algorithmic}
\end{algorithm}

where, $ u_{k} \rightarrow \mathbb{R}_{+} : u_{k} \in [1, 2]$ and is the
bounding constant that ensures the reservation price within certain
limits and is dependent upon the customer.

% *****************************************************
%
%   Old abstract
%
% *****************************************************

In this paper we describe a fictional (but realizable) business model
which profits from legitimate price gouging in a busy market. This
risk-free trade benefits from a competitive market place where our agent
acts as an arbitrageur. It is not physically bartering for any
commodity, rather for the utility pertaining the information of seller
who has the merchandise for a nominal or minimal retail. We perform
experiments and conclude that by adapting adroitness negotiation skills,
an arbitrageur (agent) can gain substantial profits by maneuvering the
price discrepancies in a market.

% *****************************************************
%
%   Older from Saad Oct 6
%
% *****************************************************

% *****************************************************
%
%   Old Introduction
%
% *****************************************************
\section{Introduction} 


As a focus for the development of ubiquitous computing technologies in
urban area, i.e., city is framed as a source of problems to be resolved.
These problems related to location, resource identification, and access
to such resources \cite{williams2008:urbane}. The emerging trend in
urban computing towards generation of applications is taking the
maneuverability in the city not as a problem to be overcome but as the
source of mutual benefits to be gained from the provided interactional
opportunities \cite{bassoli2007:underground}.

Collaborative information sharing in urban life facilitated by recent
context-aware applications is helping people to navigate their
surroundings in different ways, such as, entertainment and food (e.g.
nearest preferred mexican restaurant) \cite{dourish2010:cultural}. To
facilitate the people in urban life, a keen set of certain observations
is requierd. Observations of a particular place exhibiting everyday
urban activity gives a more authentic understanding about the importance
of its role within urban life. One of those activities includes trading
and bargaining scenarios which has made strong impact on research in
social networks for negotiations.

A good deal of research has be done in the area of bragaining mechanisms
in the field of agent systems and economics. The foundation for
alternating-offer bargaining laid by St$\dot{a}$hl
\cite{stahl1972:bargaining} has been nurtured significantly after the
literature provided by Rubinstein. Rubinstein's alternating offers
\cite{rubinstein1982:perfect} is simple enough to be characterized
allowing the both parties to use of their moves by accepting an offer or
doing a counter-offer. In this regard various tactics have evoloved with
time, e.g., behavioral tactics, time-dependent tactics etc
\cite{kraus2001:strategic}. Tactics employed by agents help them reach
at a point of agreement, mostly favouring their point of interest.

In this paper we provide a decision making framework of bilateral
negotiation process engaging a client and an agent, for location
based-service that facilitates a user through urban computing services.
Our approach focuses on different tactics to provide a balance in the
levels of information utility and negotiation price for a location-based
service. The primary contributions of this paper are:

\begin{itemize}
\item model for urban computing negotiation

\item simple tactics involving learning computations for evaluation of
opponent behvaior

\item to define and evaluate scenario for urban location-based
information which plays a significant role in facilitating everyday
life activities.

\end{itemize}


A real-world example in urban area is one depicting an alternating offer
negotiation between a client and a service provider over the price and
the amount of a service (in our case which is gas price information).
For the motivation of our research consider the diagram in Figure
\ref{fig:Motivation}.   

\begin{figure}[h!]

\centerline{
\includegraphics[width=3.25in]{Figures/Motivation} } 

\caption{Example of Gas Market Application} 

\label{fig:Example} \end{figure}

A client while on his way to home is around Lake Deeks. Observing car's
gas tank, he feels a need to have a full tank refill. The car's tank
capacity is twenty gallons. Now as shown in the Figure
\ref{fig:Motivation} the client has an idea that there are couple of gas
stations around and if he goes to the cheapest gas station, he would
definitely save some dollars. Keeping this in mind, the client opens the
location-aware application, which provides the location with cheapest
rate. Here, the client might be prompted by service provider to disclose
his location. The client wishes to access information, yet obfuscating
his exact location (due to privacy concerns). The service provider,
based on the provided location-information from user, evaluates the
cheapest gas station and informs the client that it can save few
dollars. As seen in Figure \ref{fig:Motivation} the cheapest gas station
has gas-price of \$2.73/gallon whereas another nearby station has
\$2.83/gallon. So the service provider informs the client that it has to
pay few cents if he needs the information. Based on the provided
argument by service-provider, the client starts to negotiate with the
service provider for the location-based information.

This simple scenario provides an intuitive example of negotiations in
urban location-based services. In such situations it is possible to
receive high-quality information services while negotiating for the
optimum minimal price.

% *****************************************************
%
%   Old Urban life framework
%
% *****************************************************
\section{Urban Life Framework}

%\textit{An individual`s plans must be organized in time to reflect the
%time-slots available for different kinds of activities}

Aggregated activities of individual's characterize the behavior of a
society and is therefore an important component in the urban-framework
generation \cite{bhat2004:intershopping} \cite{schönfelder2006:urban}.
For the urban activity pattern generation, we focused on some common
outdoor activities of an individual living in urban environment. The
designed framework emphasizes travel as a necessity, being derived from
the daily life activities.

Some constraints were introduced in the activity generation patterns
introduce uniqueness among different individuals. The constraints
confined individual's activities in certain spatial and temporal bounds
to avoid conflict of shared of time slots at same spatial paths.

We use term "event" as the start of an activity bounded by an interval.



% *****************************************************
%
%   Old Negotiation Strategy
%
% *****************************************************
\section{Negotiation Strategy}
The human behavior in non-complex negotiation models is no sweat, as it
is normally inclined towards maximizing self-profit. In other words, it
adapts itself to deals with beneficial output. Being fully rational
would require a human to have a unlimited intellective and mental
abilities \cite{selten2001:bounded} while dealing in such negotiable
situations. Theoretically speaking, a fully rational person would be the
one, who would have the solution to all complex mathematical queries and
is able to handle the complex situations with a sound solution set. In
real life humans have certain cognitive limitations which restricts the
solution set to a limited set of mathematical operations. Modern
psychology tells that humans are good at matching or recognizing those
patterns or behavior that result into evolutionary benefits
\cite{arthur1994:inductive}.

% *****************************************************
%
%   Old Negotiation Policy Model
%
% *****************************************************
\section{Negotiation Policy Model}
Decision alternatives for a client are not complex. The simplest case of
client satisfaction would be any deal within its reservation price. The
client decision also may be dependent upon the the compelling reasons
the server initially gives the client to buy information. Depending upon
the persuasive nature of the GasMarket Server, such as informing the
client with profit margin of cheapest gas per gallons, the client might
go bit beyond its reservation price.

The decision making process for client is the maximization of its
utility by adapting to the averaging pattern of the GasMarket server.
These previous negotiations are used by the client to calculate new
offers.



%\begin{equation} P(x) = \frac{1}{{\sigma \sqrt {2\pi } }}e^{{{ - \left(
%{x - \mu } \right)^2 } \mathord{\left/ {\vphantom {{ - \left( {x - \mu }
%\right)^2 } {2\sigma ^2 }}} \right. \kern-\nulldelimiterspace} {2\sigma
%^2 }}} \label{eqn:clientmodel} \end{equation}


% *****************************************************
%
%   Old Adaptive Learning
%
% *****************************************************
\section{Adaptive Learning}

The art of negotiation, along with the skills of negotiator are a
well-defined domain of utility information. Information, such as, demand
and its priorities, i.e., what must be get, what could get or should
get. The longer the contact period of a negotiation the richer and more
refined in context it gets. Here, adaptive learning for decision
modeling acts as a powerful tool to evaluate various scenarios.
Bilateral negotiation in our scenario being a sequential series of
bargains having no such concept of predicting the best moves by a human.
Human nature is rarely random, so instead of predicting the posterior
deals, the service provider evaluates the current trend of clients`
behavior using negotiation history. Therefore, for assessing the
likelihood of a specific behavior the adaptive learning features
provide an edge over more traditional stochastic modeling and
optimization techniques.

% *****************************************************
%
%   Old Framing Benefits and Motivating Hope
%
% *****************************************************
\section{Framing Benefits and Motivating Hope}

The service provider knows the profit margin(benefits) the client would
have if client opts for the cheapest stations. The service provider
frames the utility of the client in form of \textit{aspiration levels},
which itself is dependent upon the \textit{amount of hope} it wants to
give to the client. It can reduce its split share of profits(benefits)
and increasing \textit {level of aspiration} by giving more benefits at
low deals. \textit{Aspiration levels} are set by the service provider
keeping in view maximization of utilities for gaining more profits. If
the service provider feels a need to having more profits, then it
greedily splits the share of \textit{benefits} giving low aspiration
level to the clients. The \textit{aspiration levels} itself are dynamic
as the negotiation progresses. The service provider might raise the
aspiration level of a client if it find more alternatives from other
client for increasing benefits . So for giving the client more
\textit{hope}, the service provider starts the negotiation in round
\textit{n+1} with an initial deal that is 20\% more than the deal on
which previous negotiation ended. Also for boosting \textit{hope} the
service provider avoids offering some initial high deals and then
plunging with big steps. This also helps in avoiding more economic loss
in negotiations.



Lets have two different cases with same client. This
client sets \$3.99 as upper-limit, i.e, it is not willing to pay more
than \$3.99.

\vspace{3 mm}
\noindent\textbf{Case I-Small concession step, low initial deal}\\
\noindent The service provider makes an initial deal of \$5
with concession steps of 20 cents. After six rounds the total concession
is \$1.20. The deal is made as clients`  \textit{level of impatience}
was good enough seeing \$5 as initial offer and it negotiated till end.

\vspace{3 mm}
\noindent\textbf{Case II-Large concession steps, high initial deal}\\ \noindent
Now if an initial deal of \$7.5 is made, this might make a case of
\textit{Take it or leave it} for the client. Even though client has no
idea about the concession steps service provider might make, still its
\textit{level of impatience} might be lowered and negotiation might be
broken at first step. 

Suppose in Case II, the end result was same as agreement but the
concession steps made by service provider were of 70 cents (50 cents
more than case I). So, after same number of rounds (as of Case I) the
service provider loses 20cents in Case-II it loses 70 cents. And if
service provider sticks with monotonic concession strategy of Case-II ,
then after \textit{n} negotiation the loss ratio to Case-I is quite
high. For instance, if the above senario holds true for \textit{n}
negotiations, the loss turns out to be $3.5n$ more in Case I. 

Also, the client is the first one who gives initial deal. Its because if
the service provider states its needs first, it might lead the client to
argue (with unexpected aspiration level) or might even cause the
breaking of negotiation, as usually humans think that the first deal is
your most preferred and final deal, especially if they are inexperienced
at bargaining.

%Gamble \& risk taking to explore
%For example, give subjects $10 in advance, then ask them whether they would
%choose a certain loss of $5 (for a net gain of $5) or flip a coin and lose either $10
%or 0, depending on the outcome. Those subjects choose to gamble more frequently
%than subjects who are given nothing and asked to choose between gaining $5 or
%flipping a coin with $10 and 0 outcomes (Tversky and Kahneman, 1992).
%\cite{camerer1997progress}




% *****************************************************
%
%   Old Negotiation Protocol
%
% *****************************************************

The subject of negotiation is the piece of information associated with
cheapest gas price. In the modeled system, the customer contacts the
system when it has a need for refill. Hence, the negotiation process is
initiated by the customer, where the customer gives the initial price for
the information after an affirmative response from GPIT. Naturally,
human behavior is inclined towards maximizing self-profit and same would
be case as of GPIT for aggrandizing profits.

The gas price distribution negotiation takes place as follows. An agent
$c_{i} \in \{c_{1} \cdots c_{n}\}$ contacts the GPIT $s$. For
every negotiation $\mathcal{X}^{m}_{c \leftrightarrow s}$, let there be
a sequence of \textit{n} offers, where $\mathcal{X}^{m}_{c
\leftrightarrow s} = \{x^{1}_{c \rightarrow s} , x^{2}_{s \leftarrow c}
\cdots x^{n}_{c \leftrightarrow s}\}$. The deal after $n$ offers is
denoted by $x^{n}_{c \leftrightarrow s}$. Each agent ($c_{i}, s$) has
preferences over a sequence of deals outcome that is controlled by three
factors, i.e, initial offer, conflict offer and concession rate
$\delta_{i}$. With each deal is associated an agent $i's$ preference
$u^{i} : \{u^{i}_{min} , u^{i}_{max}\} \rightarrow \mathbb{R}$ and
concession rate $\delta_{n}^{i} \in (0, 0.5]$. The concession rate
$\delta$ varies from customer to customer and is a variable dependent
upon season(of the year). A deal is a pair $(p, d)$ where $p$ is the
piece of information associated with the cheapest gas station and $d$ is
the money that customer pays to GPIT for it. The agreement money $d$ is
confined by the preference of the customer and GPIT, i.e.,
$u^{c}_{max} \leq d \leq u^{s}_{min}$. The message format for
negotiation is as follows:

\begin{verbatim}
is-information available?
(from customer-agent, to-GPIT, negotiation initiation)  
\end{verbatim}

\noindent This is used in the context when customer requires the
information from GPIT and it waits for an affirmative response. GPIT
explores the domain of available information and responds whether it
wants to negotiate or not.

\begin{verbatim}
price-for-information
(from-agent, to-agent, offer)  
\end{verbatim}

\noindent This message contains the offer evaluations during negotiation
process. If it is used as first offer from either of the agents, it
corresponds to the willingness of a agent for a piece of information

\begin{verbatim}
price-for-information-with-benefits
(from-GPIT, to-agent, offer, benefit)  
\end{verbatim}

\noindent GPIT informs the customer about the benefits that he/she may
get by purchasing the information. This format of message is used by
GPIT to entice the customer by portraying more benefits. This is an
information tactic used by GPIT for increasing its profit, i.e., to
increase the probability that customer may purchase the information for
higher price.

\begin{verbatim}
negotiation-termination
(from-agent, to-agent, offer, deal-status)  
\end{verbatim}

\noindent This type of message is sent from one agent to the other when the
negotiation is terminated. It indicates the status of terminated
negotiation, i.e., whether it was terminated as deal-made or
deal-broken.
% *****************************************************
%
%   Old Argumentation
%
% *****************************************************

\subsection{Framing Benefits and Motivating Hope} 

Humans, on average, show more acceptance to negotiate for information
that gives them \textit{hope}. Hope is a motivational function of the
customer that is dependent upon the persuasive nature of GPIT. The
behavior of GPIT is selfish, so it frames the negotiation is such a way
that customer shows more willingness to buy the information. This leads
to importance of framing a normal negotiation into benefited-negotiation
for the customer. Hence, even if the offer from GPIT is more than
reservation price for user, i.e., $x^{n}_{s \rightarrow c} >
u^{c}_{max}$, the user still pays for the information if there is some
benefit information appended with the original piece of information.

For modeling benefits, we assume the cheapest gas station is not always
the same. Because otherwise, the customer can refill from same station
with no benefits. Let $\sigma_{max}$ be the price of the gas at
customers' current location and $\sigma_{min}$ be the price of the gas
at cheapest station. For a refill of $\rho \in \mathbb{R}_{+}$ liters,
the benefits $\psi$ by buying the information is $\rho . (\sigma_{max} -
\sigma_{min})$. Hope $\mathcal{A}_{c}(\psi)$ is given as

\begin{equation}
\mathcal{A}_{c}(\psi) = \Big\lfloor \frac{\psi} {k \cdot (x^{n}_{s \rightarrow c} -
u^{c}_{min})}  \Big\rfloor \end{equation}

where $k = rand(1,5)$ is a random number and ensures the fact that the
customer is not always desirous for benefited deals. For a
benefited-deal with $\psi \rightarrow \mathbb{Z} : \mathcal{A}_{c}(\psi)
\geq m \in [1, \infty)$ is a proposition that customer takes into
account if there is a conflict offer. The outcome of a benefited-deal is
given as \[ \begin{cases} \text{ACCEPT} & \text{iff }
\mathcal{A}_{c}(\psi) \geq 1 \text{ }\land \text{ }x^{n}_{s \rightarrow
c} > u^{c}_{max} \\ \text{REJECT} & \text{otherwise} \end{cases} \]

% *****************************************************
%
%   Old Promotional Offer
%
% *****************************************************
\subsection{Promotional offer}

We have seen that the negotiation strategy of both the client and the
GPIT is dependent on statistical information about the benefits of past
{\em successful} negotiations. To allow such a set to be acquired, the
GPIT can deploy a strategy frequently used in economical models where
repetitive buyers are expected: it announces a {\em promotional deal}
through which the user can form its historical database, form an
estimate of possible benefits, and then become a more informed customer.

FIXME: IT IS NOT CLEAR FOR ME WHETHER THAT GRAPH IS WORTH SHOWING.


The GPIT initiates the promotional offer during the inception period of
its business. During this season the GPIT gives information for free.
This helps GPIT to smooth out the initial phase of learning process as
explained in Section \ref{sec:agentdecision}. During this offer, the
GPIT asks the customer to asset the worth of information by remarking
with the amount he would pay for cheapest gas information. This
agreement is mutual exchange of information only with no costs involved,
i.e., ($u^{c}_{p}, p$). The customer provides its estimated price of
information $u^{c}_{p} = \text{rand} \Big(\mathcal{N}(\mu,
\sigma^{2})\Big)$ where $\mu = \langle \overline{u^{c}_{min},
u^{c}_{max}} \rangle \text{ and } \sigma^{2} = 1$. The GPIT provides the
cheapest gas station information $p$. Therefore, the cost of promotional
deal is $cost(\mathcal{X}^{m, p}_{c \leftrightarrow s}) = 0$. The
response of customer $u^{c}_{p}$ to GPIT promotional deal is shown in
Figure \ref{fig:PromotionalOffer}.

\begin{figure}[ht!]
\centerline{
\includegraphics[width=3.75in]{Figures/PromotionalOffer} }

\caption{Client's Promotional Offer Response} 

\label{fig:PromotionalOffer} \end{figure}



==> terminology.tex <==
\section{Terminology and Notations}

\begin{center}
\begin{tabular}{|c|l|}
\hline $\mathcal{X}^{m}_{c \leftrightarrow s}$& Negotiation between client and server \\
\hline ${x}^{n}_{a \rightarrow b}$ & $n$th offer from agent $a$ to agent $b$ \\
\hline $cost(\mathcal{X}^{n}_{c \leftrightarrow s})$ & Cost of the agreed deal in negotiation $n$ \\
\hline $c_{max}^{u}$ & Maximum limit on initial deal by user \\
\hline $u^{c}_{max}, u^{c}_{min}$ & Conflict offer and initial offer of client \\
\hline $u^{s}_{max}, u^{s}_{min}$ & Initial offer and conflict offer for server \\
\hline $u^{c}_{p}$ & Promotional offer response from user\\ 
\hline $\delta_{n}^{i}$ & Concession rate of the agent \textit{i} during deal \textit{n}\\
\hline $\psi$ & Benefits- From the server\\
\hline $\mathcal{A}_{c}(\psi)$ & Hope- Function of client\\
\hline $\phi^{n}(r_{s})$ & Exponential Moving Average for \textit{nth deal}\\
\hline $\alpha$ & EMA weight\\
\hline $r_{s}$ & EMA weighting control factor\\
\hline $\varphi$ & Moving Average Convergence Divergence\\
\hline
\end{tabular}
\end{center}


==> urban.tex <==
\subsection{Modeling of client travel patterns}

We model the travel pattern of a customer who resides in Orlando. In
Orlando the buildings are usually at distant and people prefer to travel
by cars. For modeling the car consumption, we used a typical car with
gas tank of fifteen gallons and average gas consumption of twenty miles
per gallon. For describing an individual's travel pattern we use the
data structure as shown in Listing \ref{fig:urbanpattern}. The data is
based on recurring events in daily life of a client, where his work
habits are from 8am to 5pm (on average) in weekdays.

For generation of realistic scenario the path planning was carried out
using Google Maps. We selected those routes which had relatively heavy
traffic patterns. The jobs places and residential area were also taken
into consideration. Probability of event occurrence was introduced to
simulate the recurrence of execution of certain travel intervals. The
probability of an event generation for activities such as shopping was
low on weekdays and high on weekends.


\lstset{caption=Sample of Urban-life Activity Pattern,label=fig:urbanpattern} 
\lstinputlisting{Figures/exscen.txt}

\noindent For generation of overall activity patterns, a scenario
generator was created. The input parameter to the scenario generator
were the gas stations, the average price curve, variance between
different stations. The output of generator was a list of customers and
the generated travel paths. The generator using a transition matrix
$A(L, d, t)$ used to select next location based on the current location
$L$, day of week $d$, and the time $t$. After the transitions selection,
the map querying services were invoked to find out the gas stations in
the spatial path. Google Maps queries returned the data in KML format,
from where required data was parsed out.

\subsection{Event Generation}

Listing \ref{fig:urbanpattern} shows a list of various events for each
client. Every event \textit{E(u)} of a client \textit{u} is composed of
event-type, time-stamp and distance traveled.
\vspace{3 mm}

\noindent \textbf{Event Type}

\noindent The event can be from one of the following types

\begin{enumerate}

\item \textbf{Departs} This indicates the event when an individual
leaves a particular location

\item \textbf{Arrives} This event is triggered at the arrival of client
at particular location

\item \textbf{Sees} This event shows the occurrence of an event, when a
person sees a gas station

\item \textbf{Needs} This is an internal event generated during
simulation. And it is triggered when client is almost out of gas. For
simulation purposes, this event was generated when client's car, gas
tank was below two gallons.

\end{enumerate}
%\vspace{3 mm}
\noindent \textbf{Location}

\noindent The travel path of an individual from home origin to work
(destination) is shown in Figure \ref{fig:Scenario}. The real locations
are classified as Work-location (W), Shopping-location (S) and
Residential-location (R).

\vspace{3 mm}
\noindent \textbf{Time Stamp}

\noindent Each day in the \textit{DATE} has a duration of 24000ms. This
makes one simulated hour equivalent to 100ms.

\vspace{3 mm}
\noindent \textbf{Travel Distance}

\noindent The distance traveled was calculated using Google Maps queries.
The distance traveled was used for calculating the gas consumption
between occurrence of different activities. 





==> userModeling.tex <==
\section{Negotiation protocol and strategy}
\label{sec:NegotiationProtocol}

In this section we describe the procedure for the negotiation of the information. Let us consider a customer who is driving according to his lifestyle, gradually exhausting the fuel in his car. When the quantity of fuel drops below a certain level the customer will look for a gas station to refuel. The current location and planned path of the customer has a significant impact on which gas stations are the best refuelling choice. 

To save on the cost of fuel by choosing the optimal gas station, the driver contacts the GPIT, sends its location, planned path, and requests information about the optimal gas station at the same time making a price offer $x^1_{c \rightarrow s}$. The GPIT calculates this information and replies with a counter offer $x^2_{c \leftarrow s}$. 

The negotiation will consist of a series of exchanged offers $\mathcal{X}^{m}_{c \leftrightarrow s} = \{x^{1}_{c \rightarrow s} , x^{2}_{s \leftarrow c} \cdots x^{n}_{c \leftrightarrow s}\}$. If the negotiation was successful, it will conclude with a deal $x^{n}_{c \leftrightarrow s}$. In this case, the client will pay $x^{n}_{c \leftrightarrow s}$ dollars to the GPIT, and the GPIT will deliver the information to the client (who will use it to choose the gas station to refuel). If the negotiation concludes with the conflict deal, no money or information is exchanged and the client will refuel at the first gas station on its projected path. 

The negotiation strategy of the client is a monotonic, uniform concession with reservation price. The first offer made by the client is at $u_{min}$, it will uniformly concede with a concession rate $\delta \in (0, 0.5]$ until it reaches the reservation price $u_{max}$, at which point it will insist on its offer. A full negotiation round without concession from either side breaks the negotiation. The GPIT is using a similar strategy. With this strategy, the deal is $x^{n}_{c \leftrightarrow s} \in (u_{min} , u_{max}]$


HERE WE ARE

TO MY MIND WHAT REMAINS IS NOT NECESSARY, BUT I DONT UNDERSTAND THE STORY WITH THE EVALUATIONS

The subject of negotiation is the piece of information associated with
cheapest gas price. In the modeled system, the customer contacts the
system when it has a need for refill. Hence, the negotiation process is
initiated by the customer, where the customer gives the initial price for
the information after an affirmative response from GPIT. Naturally,
human behavior is inclined towards maximizing self-profit and same would
be case as of GPIT for aggrandizing profits.

The gas price distribution negotiation takes place as follows. An agent
$c_{i} \in \{c_{1} \cdots c_{n}\}$ contacts the GPIT $s$. For
every negotiation $\mathcal{X}^{m}_{c \leftrightarrow s}$, let there be
a sequence of \textit{n} offers, where $\mathcal{X}^{m}_{c
\leftrightarrow s} = \{x^{1}_{c \rightarrow s} , x^{2}_{s \leftarrow c}
\cdots x^{n}_{c \leftrightarrow s}\}$. The deal after $n$ offers is
denoted by $x^{n}_{c \leftrightarrow s}$. Each agent ($c_{i}, s$) has
preferences over a sequence of deals outcome that is controlled by three
factors, i.e, initial offer, conflict offer and concession rate
$\delta_{i}$. With each deal is associated an agent $i's$ preference
$u^{i} : \{u^{i}_{min} , u^{i}_{max}\} \rightarrow \mathbb{R}$ and
concession rate $\delta_{n}^{i} \in (0, 0.5]$. The concession rate
$\delta$ varies from customer to customer and is a variable dependent
upon season(of the year). A deal is a pair $(p, d)$ where $p$ is the
piece of information associated with the cheapest gas station and $d$ is
the money that customer pays to GPIT for it. The agreement money $d$ is
confined by the preference of the customer and GPIT, i.e.,
$u^{c}_{max} \leq d \leq u^{s}_{min}$. The message format for
negotiation is as follows:

\begin{verbatim}
is-information available?
(from customer-agent, to-GPIT, negotiation initiation)  
\end{verbatim}

\noindent This is used in the context when customer requires the
information from GPIT and it waits for an affirmative response. GPIT
explores the domain of available information and responds whether it
wants to negotiate or not.

\begin{verbatim}
price-for-information
(from-agent, to-agent, offer)  
\end{verbatim}

\noindent This message contains the offer evaluations during negotiation
process. If it is used as first offer from either of the agents, it
corresponds to the willingness of a agent for a piece of information

\begin{verbatim}
price-for-information-with-benefits
(from-GPIT, to-agent, offer, benefit)  
\end{verbatim}

\noindent GPIT informs the customer about the benefits that he/she may
get by purchasing the information. This format of message is used by
GPIT to entice the customer by portraying more benefits. This is an
information tactic used by GPIT for increasing its profit, i.e., to
increase the probability that customer may purchase the information for
higher price.

\begin{verbatim}
negotiation-termination
(from-agent, to-agent, offer, deal-status)  
\end{verbatim}

\noindent This type of message is sent from one agent to the other when the
negotiation is terminated. It indicates the status of terminated
negotiation, i.e., whether it was terminated as deal-made or
deal-broken.


